Multi-Objective Few-shot Learning for Fair Classification

In this paper, we propose a general framework for mitigating the disparities of the predicted classes with respect to secondary attributes within the data (e.g., race, gender etc.). Our proposed method involves learning a multi-objective function that in addition to learning the primary objective of predicting the primary class labels from the data, also employs a clustering-based heuristic to minimize the disparities of the class label distribution with respect to the cluster memberships, with the assumption that each cluster should ideally map to a distinct combination of attribute values. Experiments demonstrate effective mitigation of cognitive biases on a benchmark dataset without the use of annotations of secondary attribute values (the zero-shot case) or with the use of a small number of attribute value annotations (the few-shot case).

==> tabfigdefs/contingency.tex <==
\begin{table}[!t]
\centering
\small
\begin{tabular}{@{}l@{~~}l@{~~}c@{~~}c@{~~}c@{}}
\toprule
Emotion & Attribute &  & \multicolumn{2}{c}{$|\mathbb{I}(\hat{y}=c)|$}\\
\cmidrule(r){4-5}
($c$) & ($z$) & $|\mathbb{I}(y=c)|$ & BALR & BACP-L2X \\
\midrule
\multirow{2}{*}{$c=$ Fear}& $z=$ Male & 150 & 30 & 35 \\
& $z=$ Female & 260 & 140 & 122 \\
\midrule
\multirow{2}{*}{$c=$ Fear} & $z=$ Caucasian & 100 & 100 & 90 \\
& $z=$ African-American & 60 & 60 & 60 \\
\midrule
\multirow{2}{*}{$c=$ Anger} & $z=$ Female & 110 & 110 & 110 \\
& $z=$ Male & 150 & 150 & 140\\
\bottomrule
\end{tabular}
\caption{Contingency table of the reference emotion labels vs. the predicted labels for different attribute values. $\mathbb{I}(y=c)$ indicates the set of instances where the reference label's ($y$) value is $c$ (e.g. fear), and similarly $\mathbb{I}(\hat{y}=c)$ indicates the set for which the predicted emotion category ($\hat{y}$) is $c$.}
\label{tab:contingency}
\end{table}


==> tabfigdefs/epsilon-K-sensitivity.tex <==





